Maximizing Non-Monotone Submodular Functions over Small Subsets: Beyond $1/2$-Approximation

In this work we give two new algorithms that use similar techniques for (non-monotone) submodular function maximization subject to a cardinality constraint. The first is an offline fixed parameter tractable algorithm that guarantees a $0.539$-approximation for all non-negative submodular functions. The second algorithm works in the random-order streaming model. It guarantees a $(1/2+c)$-approximation for symmetric functions, and we complement it by showing that no space-efficient algorithm can beat $1/2$ for asymmetric functions. To the best of our knowledge this is the first provable separation between symmetric and asymmetric submodular function maximization.

==> abstract.tex <==
\begin{abstract}
In this work we give two new algorithms for (non-monotone) submodular function maximization subject to a cardinality constraint.

The first is an offline fixed parameter tractable algorithm that guarantees a $0.51$-approximation for all submodular functions. 

The second algorithm works in the random-order streaming model. It guarantees a $0.51$-approximation for  {\em symmetric} functions, and we complement it by showing that no space-efficient algorithm can beat $1/2$ for asymmetric functions. To the best of our knowledge this is the first provable separation between symmetric and asymmetric submodular function maximization.
\end{abstract}
